Playable Video Generation

This paper introduces the unsupervised learning problem of playable video generation (PVG). In PVG, we aim at allowing a user to control the generated video by selecting a discrete action at every time step as when playing a video game. The difficulty of the task lies both in learning semantically consistent actions and in generating realistic videos conditioned on the user input. We propose a novel framework for PVG that is trained in a self-supervised manner on a large dataset of unlabelled videos. We employ an encoder-decoder architecture where the predicted action labels act as bottleneck. The network is constrained to learn a rich action space using, as main driving loss, a reconstruction loss on the generated video. We demonstrate the effectiveness of the proposed approach on several datasets with wide environment variety. Further details, code and examples are available on our project page willi-menapace.github.io/playable-video-generation-website.

==> bair_breakout_reconstruction.tex <==
\begin{table}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    
    \begin{tabular}{l@{\hskip 1mm}ccc}
         & $t=1$ & $t=5$ & $t=10$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/original/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/original/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/original/00016.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp/00016.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp_plus/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp_plus/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/savp_plus/00016.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/ours/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/ours/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/breakout_reconstruction/ours/00016.png} \\

         
    \end{tabular}
    \quad
    \begin{tabular}{l@{\hskip 1mm}ccc}
         & $t=1$ & $t=5$ & $t=10$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00016.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00016.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00016.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00016.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstruction results on the \emph{Atari Breakout} (left) and \emph{BAIR} (right) datasets. \willi{comment for bair it is seq 16}}
    \label{fig:qualitative_bair_breakout_reconstruction}
\end{table}

==> bair_reconstruction.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}cccccccccc}
         & $t=1$ & $t=2$ & $t=3$ & $t=4$ & $t=5$ & $t=6$ & $t=7$ & $t=8$ & $t=9$ & $t=10$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00008.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00010.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00013.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00014.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/original/00016.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00008.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00010.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00013.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00014.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp/00016.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00008.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00010.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00013.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00014.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/savp_plus/00016.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} & \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00007.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00008.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00010.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00011.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00013.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00014.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_reconstruction/ours/00016.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Sample video sequences generated from the same starting frame with all different learned  discrete action inputs.}
    \label{fig:tennis_action_unrolls}
\end{table*}

==> supplementary_plots/action_space_visualizations.tex <==
\begin{figure*}
\centering
\resizebox{\linewidth}{!}{
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[trim=60 40 130 50,clip,width=1\linewidth]{supplementary_resources/action_space_bair.pdf}
  \caption{\emph{BAIR}}
  \label{fig:action_space_bair}
\end{subfigure}%
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[trim=60 40 130 50,clip,width=0.8\linewidth]{supplementary_resources/action_space_breakout.pdf}
  \caption{\emph{Atari Breakout}}
  \label{fig:action_space_breakout}
\end{subfigure}
\begin{subfigure}{.33\textwidth}
  \centering
  \includegraphics[trim=60 40 130 50,clip,width=1\linewidth]{supplementary_resources/action_space_tennis.pdf}
  \caption{\emph{Tennis}}
  \label{fig:action_space_tennis}
\end{subfigure}
}
\caption{Visualizations of the learned space of \emph{action directions} $d_t$ with corresponding \textit{action direction centroids} $\{c_k\}_{k=1}^{K}$, grouped by action.}
\label{fig:action_space}
\end{figure*}

==> supplementary_plots/action_unrolls/bair_breakout_action_unrolls.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{

    \setlength\tabcolsep{0.5pt}
    \footnotesize

    \begin{tabular}{l@{\hskip 0.7mm}ccccccc}
         
         & Action 1 & Action 2 & Action 3 & Action 4 & Action 5 & Action 6 & Action 7 \\
         
         \rotatebox{90}{\setlength{\thickmuskip}{0mu}\hspace{6mm}$t=6$\hspace{11.5mm}$t=4$\hspace{11.5mm}$t=2$\hspace{11.5mm}$t=0$} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_0.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_1.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_2.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_3.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_4.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_5.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/0_6.png}} \\
         
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_0.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_1.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_2.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_3.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_4.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_5.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/bair_action_unrolls/2d_action_density_action_6.pdf} \\
         
         
    \end{tabular}
    \quad
    \begin{tabular}{l@{\hskip 0.7mm}ccc}
     
         & Action 1 & Action 2 & Action 3 \\
         
         \rotatebox{90}{\setlength{\thickmuskip}{0mu}\hspace{6mm}$t=6$\hspace{11.5mm}$t=4$\hspace{11.5mm}$t=2$\hspace{11.5mm}$t=0$}
         &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/breakout_action_unrolls/2_0.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/breakout_action_unrolls/2_1.png}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/breakout_action_unrolls/2_2.png}} \\
         
         %& \includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/breakout_action_unrolls/2d_action_density_action_0.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/breakout_action_unrolls/2d_action_density_action_1.pdf} &
         %\includegraphics[trim=65 85 52 80,clip,width=0.2\columnwidth]{resources/breakout_action_unrolls/2d_action_density_action_2.pdf} \\
         
    \end{tabular}
    }
    \captionof{figure}{Videos generated by \methodname~on the \emph{BAIR} (left) and on the \emph{Atari Breakout} (right) datasets. We generate a sequence for each learned action by repeatedly inputting the current action starting from the same initial frame. In all datasets, the model learns actions that correspond to movement on each axis. Additional videos are shown in the corresponding section of the \href{run:./main.html}{main.html} page.}
    \label{fig:bair_breakout_action_unrolls}

\end{table*}

==> supplementary_plots/action_unrolls/tennis_action_unrolls.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0.5pt}
    \scriptsize
    \begin{tabular}{l@{\hskip 0.7mm}ccccccc}
         
         & Action 1 & Action 2 & Action 3 & Action 4 & Action 5 & Action 6 & Action 7 \\
         
         \rotatebox{90}{\setlength{\thickmuskip}{0mu}\resizebox{30mm}{!}{\hspace{2mm}$t=8$\hspace{4mm}$t=6$\hspace{4mm}$t=4$\hspace{4mm}$t=2$\hspace{4mm}$t=0$}} &
         \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_0.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_1.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_2.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_3.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_4.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_5.png}} & \setlength{\fboxsep}{0pt}\fbox{\includegraphics[width=0.2\columnwidth]{resources/tennis_action_unrolls/0_6.png}} \\
         
         %& \includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_0.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_1.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_2.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_3.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_4.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_5.pdf} &
         %\includegraphics[trim=62 85 49 80,clip,width=0.2\columnwidth]{resources/tennis_action_unrolls/2d_action_density_action_6.pdf} \\
         
         
    \end{tabular}
    }
    \captionof{figure}{Videos generated by \methodname~on the \emph{Tennis} dataset. We generate a sequence for each learned action by repeatedly inputting the current action starting from the same initial frame. The model learns actions that correspond horizontal (Act. 4 and Act. 7) and vertical player movement (Act. 2 and Act. 3), no movement (Act. 6), and ball hitting (Act. 1, Act. 5). Additional videos are shown in the corresponding section of the \href{run:./main.html}{main.html} page.}
    \label{fig:tennis_action_unrolls}
\end{table*}

==> supplementary_plots/bair_reconstruction_111.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/111/00029.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.94}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/111/00029.png} \\
         
         \rotatebox{90}{\hspace{1mm}MoCoGAN+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/111/00029.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/111/00029.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/111/00029.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/111/00029.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{BAIR} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:bair_reconstruction_111}
\end{table*}

==> supplementary_plots/bair_reconstruction_117.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/117/00029.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.94}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/117/00029.png} \\
         
         \rotatebox{90}{\hspace{1mm}MoCoGAN+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/117/00029.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/117/00029.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/117/00029.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/117/00029.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{BAIR} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:bair_reconstruction_117}
\end{table*}

==> supplementary_plots/bair_reconstruction_119.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{3.5mm}Original} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/original/119/00029.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.94}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco/119/00029.png} \\
         
         \rotatebox{90}{\hspace{1mm}MoCoGAN+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/moco_plus/119/00029.png} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp/119/00029.png} \\
         
         \rotatebox{90}{\hspace{4mm}SAVP+} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/savp_plus/119/00029.png} \\
         
         \rotatebox{90}{\hspace{6mm}Ours} &
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00000.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00003.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00006.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00009.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00012.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00015.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00018.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00021.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00024.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00027.png} & 
         \includegraphics[trim=2 0 0 2,clip,width=0.2\columnwidth]{supplementary_resources/bair/ours/119/00029.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{BAIR} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:bair_reconstruction_119}
\end{table*}

==> supplementary_plots/breakout_reconstruction_0.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{0.8\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{5.5mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/0/00031.png} \\
         
         \rotatebox{90}{\hspace{2mm}MoCoGAN \cite{tulyakov2018moco}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/0/00031.png} \\
         
         \rotatebox{90}{\hspace{3mm}MoCoGAN+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/0/00031.png} \\
         
         \rotatebox{90}{\hspace{5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/0/00031.png} \\
         
         \rotatebox{90}{\hspace{6mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/0/00031.png} \\
         
         \rotatebox{90}{\hspace{7.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/0/00031.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Atari Breakout} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:breakout_reconstruction_0}
\end{table*}

==> supplementary_plots/breakout_reconstruction_11.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{0.8\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{5.5mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/11/00031.png} \\
         
         \rotatebox{90}{\hspace{2mm}MoCoGAN \cite{tulyakov2018moco}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/11/00031.png} \\
         
         \rotatebox{90}{\hspace{3mm}MoCoGAN+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/11/00031.png} \\
         
         \rotatebox{90}{\hspace{5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/11/00031.png} \\
         
         \rotatebox{90}{\hspace{6mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/11/00031.png} \\
         
         \rotatebox{90}{\hspace{7.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/11/00031.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Atari Breakout} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:breakout_reconstruction_11}
\end{table*}

==> supplementary_plots/breakout_reconstruction_36.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{0.8\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \footnotesize
    \renewcommand{\arraystretch}{0.5}
    \begin{tabular}{l@{\hskip 1mm}ccccccccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$ & $t=19$ & $t=22$ & $t=25$ & $t=28$ & $t=30$  \\
         \rotatebox{90}{\hspace{5.5mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/original/36/00031.png} \\
         
         \rotatebox{90}{\hspace{2mm}MoCoGAN \cite{tulyakov2018moco}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco/36/00031.png} \\
         
         \rotatebox{90}{\hspace{3mm}MoCoGAN+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/moco_plus/36/00031.png} \\
         
         \rotatebox{90}{\hspace{5mm}SAVP \cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp/36/00031.png} \\
         
         \rotatebox{90}{\hspace{6mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/savp_plus/36/00031.png} \\
         
         \rotatebox{90}{\hspace{7.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00015.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00018.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00021.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00024.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00027.png} & 
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/breakout/ours/36/00031.png} \\

         
    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Atari Breakout} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:breakout_reconstruction_36}
\end{table*}

==> supplementary_plots/density_plots/bair_density_plots.tex <==



\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.7}
    \begin{tabular}{l@{\hskip 0.7mm}ccccccc}
         & Action 1 & Action 2 & Action 3 & Action 4 & Action 5 & Action 6 & Action 7  \\

         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN+}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/moco_plus/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{1.8mm}SAVP\cite{lee2018savp}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP+} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/savp_plus/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{3mm}Ours} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/bair/density_plots/ours/2d_action_density_action_6.pdf} \\

    \end{tabular}
    }
    \captionof{figure}{Distribution of the displacement $\Delta$ associated with robot arm on the \emph{BAIR} dataset. Ideal distributions are different for each action and have low variance, meaning that they capture specific movements. The displacement component associated with movement on the vertical axis $z$ is not shown. While the distributions of the displacement $\Delta$ on the $x$ and $y$ axes associated with the SAVP and SAVP+ baselines are influenced by the input action, they do not successfully capture movement of the robot arm on the $z$ axis. This is reflected in the $\Delta$-\emph{MSE} score which shows that the actions learned by our model correspond to more specific movements than the ones learned by the baselines.}
    \label{fig:bair_density_plots}
\end{table*}


==> supplementary_plots/density_plots/breakout_density_plots.tex <==
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{0.43\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.7}
    \begin{tabular}{l@{\hskip 0.7mm}ccc}
         & Action 1 & Action 2 & Action 3  \\

         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco/2d_action_density_action_2.pdf} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN+}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/moco_plus/2d_action_density_action_2.pdf} \\
         
         \rotatebox{90}{\hspace{1.8mm}SAVP\cite{lee2018savp}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp/2d_action_density_action_2.pdf} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP+} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/savp_plus/2d_action_density_action_2.pdf} \\
         
         \rotatebox{90}{\hspace{3mm}Ours} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/ours/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/ours/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/breakout/density_plots/ours/2d_action_density_action_2.pdf} \\

    \end{tabular}
    }
    \captionof{figure}{Distribution of the displacement $\Delta$ associated with the player-controlled platform on the \emph{Atari Breakout} dataset. Ideal distributions are different for each action and have low variance, meaning that they capture specific movements. Differently from the baselines, our model learns actions that correspond to specific movements of the platform.}
    \label{fig:breakout_density_plots}
\end{table*}

==> supplementary_plots/density_plots/tennis_density_plots.tex <==

\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.7}
    \begin{tabular}{l@{\hskip 0.7mm}ccccccc}
         & Action 1 & Action 2 & Action 3 & Action 4 & Action 5 & Action 6 & Action 7  \\

         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{1}{MoCoGAN+}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/moco_plus/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{1.8mm}SAVP\cite{lee2018savp}} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{2.5mm}SAVP+} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/savp_plus/2d_action_density_action_6.pdf} \\
         
         \rotatebox{90}{\hspace{3mm}Ours} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_0.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_1.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_2.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_3.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_4.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_5.pdf} &
         \includegraphics[trim=60 80 60 80,clip,width=0.2\columnwidth]{supplementary_resources/tennis/density_plots/ours/2d_action_density_action_6.pdf} \\

    \end{tabular}
    }
    \captionof{figure}{Distribution of the displacement $\Delta$ associated with the player on the \emph{Tennis} dataset. Ideal distributions are different for each action and have low variance, meaning that they capture specific movements. Our model successfully conditions the movement of the player on the action, while the other baselines show limited conditioning capabilities.}
    \label{fig:tennis_density_plots}
\end{table*}


==> supplementary_plots/human_evaluation_votes/amt_votes_tables.tex <==
\begin{table}
\begin{center}

\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \emph{Hit} & \emph{Forward} & \emph{Backward} & \emph{Right} & \emph{Other} & \emph{Stay} & \emph{Left}  \\
\hline\noalign{\smallskip}
Act. 1 & 44 & 6 & 3 & 49 & 2 & 51 & 75 \\
Act. 2 & 40 & 6 & 4 & 57 & 6 & 47 & 70 \\
Act. 3 & 49 & 7 & 6 & 52 & 2 & 46 & 68 \\
Act. 4 & 46 & 7 & 3 & 48 & 3 & 49 & 74 \\
Act. 5 & 38 & 7 & 3 & 49 & 5 & 52 & 76 \\
Act. 6 & 34 & 6 & 6 & 51 & 5 & 50 & 78 \\
Act. 7 & 43 & 7 & 3 & 49 & 6 & 50 & 72 \\
\hline
\end{tabular}
\end{center}
\caption{AMT votes for MoCoGAN \cite{tulyakov2018moco} on the \emph{Tennis} dataset.}
\label{table:amt_votes_moco}
\end{table}

\begin{table}
\begin{center}

\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \emph{Hit} & \emph{Forward} & \emph{Backward} & \emph{Right} & \emph{Other} & \emph{Stay} & \emph{Left}  \\
\hline\noalign{\smallskip}
Act. 1 & 20 & 6 & 2 & 94 & 61 & 12 & 35 \\
Act. 2 & 14 & 5 & 4 & 90 & 68 & 10 & 39 \\
Act. 3 & 24 & 7 & 2 & 92 & 66 & 4 & 35 \\
Act. 4 & 22 & 6 & 2 & 90 & 68 & 5 & 37 \\
Act. 5 & 26 & 3 & 2 & 86 & 67 & 9 & 37 \\
Act. 6 & 26 & 7 & 2 & 85 & 64 & 9 & 37 \\
Act. 7 & 20 & 11 & 2 & 86 & 57 & 12 & 42 \\
\hline
\end{tabular}
\end{center}
\caption{AMT votes for MoCoGAN+ on the \emph{Tennis} dataset.}
\label{table:amt_votes_moco_plus}
\end{table}

\begin{table}
\begin{center}
\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \emph{Hit} & \emph{Forward} & \emph{Backward} & \emph{Right} & \emph{Other} & \emph{Stay} & \emph{Left}  \\
\hline\noalign{\smallskip}
Act. 1 & 50 & 15 & 27 & 25 & 10 & 45 & 58 \\
Act. 2 & 27 & 4 & 26 & 84 & 17 & 14 & 58 \\
Act. 3 & 22 & 8 & 18 & 54 & 13 & 10 & 105 \\
Act. 4 & 42 & 12 & 37 & 26 & 26 & 38 & 49 \\
Act. 5 & 19 & 7 & 26 & 81 & 25 & 20 & 52 \\
Act. 6 & 5 & 7 & 12 & 62 & 7 & 10 & 127 \\
Act. 7 & 60 & 21 & 19 & 7 & 17 & 95 & 11 \\
\hline
\end{tabular}
\end{center}
\caption{AMT votes for the SAVP \cite{lee2018savp} method on the \emph{Tennis} dataset.}
\label{table:amt_votes_savp}
\end{table}

\begin{table}
\begin{center}

\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \emph{Hit} & \emph{Forward} & \emph{Backward} & \emph{Right} & \emph{Other} & \emph{Stay} & \emph{Left}  \\
\hline\noalign{\smallskip}
Act. 1 & 30 & 16 & 13 & 83 & 19 & 19 & 50 \\
Act. 2 & 36 & 24 & 7 & 88 & 2 & 25 & 48 \\
Act. 3 & 34 & 19 & 8 & 82 & 11 & 24 & 52 \\
Act. 4 & 36 & 17 & 10 & 88 & 13 & 22 & 44 \\
Act. 5 & 31 & 18 & 13 & 87 & 17 & 16 & 48 \\
Act. 6 & 24 & 17 & 10 & 91 & 13 & 29 & 46 \\
Act. 7 & 42 & 14 & 9 & 88 & 12 & 18 & 47 \\
\hline
\end{tabular}
\end{center}
\caption{AMT votes for the SAVP+ method on the \emph{Tennis} dataset.}
\label{table:amt_votes_savp_plus}
\end{table}



\begin{table}
\begin{center}

\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{lccccccc}
\hline\noalign{\smallskip}
 & \emph{Hit} & \emph{Forward} & \emph{Backward} & \emph{Right} & \emph{Other} & \emph{Stay} & \emph{Left}  \\
\hline\noalign{\smallskip}
Act. 1 & 21 & 62 & 1 & 122 & 4 & 15 & 5 \\
Act. 2 & 6 & 203 & 2 & 17 & 1 & 0 & 1 \\
Act. 3 & 7 & 2 & 137 & 15 & 14 & 7 & 48 \\
Act. 4 & 2 & 1 & 3 & 219 & 4 & 0 & 1 \\
Act. 5 & 20 & 8 & 52 & 19 & 2 & 27 & 102 \\
Act. 6 & 20 & 16 & 8 & 22 & 1 & 111 & 52 \\
Act. 7 & 10 & 13 & 2 & 0 & 3 & 1 & 201 \\
\hline
\end{tabular}
\end{center}
\caption{AMT votes for the our method on the \emph{Tennis} dataset.}
\label{table:amt_votes_ours}
\end{table}

==> supplementary_plots/tennis_interpolation.tex <==
\begin{figure*}
\centering
\resizebox{\linewidth}{!}{
\includegraphics[width=1\linewidth]{supplementary_resources/tennis/interpolation.pdf}
}
\caption{Visualization of the last frame of sequences produced from the same initial frame with differing \emph{actions} and \emph{action variability embeddings}. The sequences in red represent pure discrete actions where, \emph{action variability embeddings} are posed to 0. For the sequences in black instead, \emph{actions} and \emph{action variability embeddings} are derived as described in Sec.~\ref{sec:action_variability_embeddings} to represent intermediate actions between the two closest discrete actions using values of the \emph{interpolation factor} of 0.3, 0.5 and 0.7. Note how the player positions depicted in the black sequences smoothly interpolate between the positions obtained with pure discrete actions, showing the capability of \emph{action variability embeddings} to capture variations on discrete actions.}
\label{fig:action_interpolation}
\end{figure*}

==> supplementary_plots/tennis_reconstruction_115.tex <==



\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.35}
    \begin{tabular}{l@{\hskip 0.7mm}cccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$  \\
         \rotatebox{90}{\hspace{0mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/115/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.6}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/115/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.7}{MoCoGAN+}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/115/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}SAVP\cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/115/00015.png} \\
         
         \rotatebox{90}{\hspace{0.5mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/115/00015.png} \\
         
         \rotatebox{90}{\hspace{1.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/115/00015.png} \\
         

    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Tennis} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:tennis_reconstruction_111}
\end{table*}


==> supplementary_plots/tennis_reconstruction_39.tex <==



\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.35}
    \begin{tabular}{r@{\hskip 0.7mm}cccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$  \\
         \rotatebox{90}{\hspace{0mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/39/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.55}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/39/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.65}{MoCoGAN+}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/39/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}SAVP\cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/39/00015.png} \\
         
         \rotatebox{90}{\hspace{0.5mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/39/00015.png} \\
         
         \rotatebox{90}{\hspace{1.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/39/00015.png} \\
         

    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Tennis} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:tennis_reconstruction_39}
\end{table*}


==> supplementary_plots/tennis_reconstruction_52.tex <==



\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.35}
    \begin{tabular}{r@{\hskip 0.7mm}cccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$  \\
         \rotatebox{90}{\hspace{0mm}Original} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/original/52/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.55}{MoCoGAN \cite{tulyakov2018moco}}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco/52/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}\scalebox{0.65}{MoCoGAN+}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/moco_plus/52/00015.png} \\
         
         \rotatebox{90}{\hspace{0mm}SAVP\cite{lee2018savp}} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp/52/00015.png} \\
         
         \rotatebox{90}{\hspace{0.5mm}SAVP+} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/savp_plus/52/00015.png} \\
         
         \rotatebox{90}{\hspace{1.5mm}Ours} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00000.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00003.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00006.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00009.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00012.png} &
         \includegraphics[width=0.2\columnwidth]{supplementary_resources/tennis/ours/52/00015.png} \\
         

    \end{tabular}
    }
    \captionof{figure}{Reconstructed sequences on the \emph{Tennis} dataset using the learned, discrete actions extracted from the original sequence as inputs.}
    \label{fig:tennis_reconstruction_52}
\end{table*}


==> tennis_reconstruction.tex <==


\begin{table}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.35}
    \begin{tabular}{l@{\hskip 0.7mm}cccccc}
         & $t=1$ & $t=8$ & $t=16$  \\
         \rotatebox{90}{\hspace{0mm}Original} & \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00000.png} &
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00007.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00015.png}  \\
         
         \rotatebox{90}{\hspace{-0.3mm}\scalebox{0.7}{MoCoGAN+}} & \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/moco_plus/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/moco_plus/00007.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/moco_plus/00015.png}  \\
         
         \rotatebox{90}{\hspace{0.5mm}SAVP+} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00007.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00015.png}  \\
         
         \rotatebox{90}{\hspace{1.5mm}Ours} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00007.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00015.png}  \\
         
         
    \end{tabular}
    }
    \captionof{figure}{Reconstruction results on the \emph{Tennis} dataset. \willi{comment it is sequence 115}}
    \label{fig:qualitative_tennis_reconstruction}
\end{table}

\begin{comment}
\begin{table*}
    \centering
    \def\arraystretch{1.0}
    \resizebox{\linewidth}{!}{
    \setlength\tabcolsep{0pt}
    \tiny
    \renewcommand{\arraystretch}{0.35}
    \begin{tabular}{l@{\hskip 0.7mm}cccccc}
         & $t=1$ & $t=4$ & $t=7$ & $t=10$ & $t=13$ & $t=16$  \\
         \rotatebox{90}{\hspace{0mm}Original} & \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00000.png} &
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/original/00015.png}  \\
         
         \rotatebox{90}{\hspace{1mm}SAVP} & \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp/00015.png}  \\
         
         \rotatebox{90}{\hspace{0.5mm}SAVP+} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/savp_plus/00015.png}  \\
         
         \rotatebox{90}{\hspace{1.5mm}Ours} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00000.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00003.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00006.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00009.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00012.png} & 
         \includegraphics[width=0.2\columnwidth]{resources/tennis_reconstruction/ours/00015.png}  \\
         
         
         
    \end{tabular}
    }
    \captionof{figure}{Sample video sequences generated from the same starting frame with all different learned  discrete action inputs.}
    \label{fig:tennis_action_unrolls}
\end{table*}
\end{comment}
